Greedy Emulators for Nuclear Two-Body Scattering

Applications of reduced basis method emulators are increasing in low-energy nuclear physics because they enable fast and accurate sampling of high-fidelity calculations, enabling robust uncertainty quantification. In this paper, we develop, implement, and test two model-driven emulators based on (Petrov-)Galerkin projection using the prototypical test case of two-body scattering with the Minnesota potential and a more realistic local chiral potential. The high-fidelity scattering equations are solved with the matrix Numerov method, a reformulation of the popular Numerov recurrence relation for solving special second-order differential equations as a linear system of coupled equations. A novel error estimator based on reduced-space residuals is applied to an active learning approach (a greedy algorithm) to choosing training samples ("snapshots") for the emulator and contrasted with a proper orthogonal decomposition (POD) approach. Both approaches allow for computationally efficient offline-online decompositions, but the greedy approach requires much fewer snapshot calculations. These developments set the groundwork for emulating scattering observables based on chiral nucleon-nucleon and three-nucleon interactions and optical models, where computational speed-ups are necessary for Bayesian uncertainty quantification. Our emulators and error estimators are widely applicable to linear systems.

==> figures/tikz/greedy_flowchart_landscape.tex <==



% Figure 4 is out of sync with the main text. Could you please make a suggestion for making the figure less of a copy of the enumerate list in the main text?






% \documentclass{article}
% \usepackage{lscape}
% \usepackage[dvipsnames]{xcolor}
% \usepackage[legalpaper, landscape, margin=2in]{geometry}
% \usepackage{tikz}
% \usepackage{bm}
\usetikzlibrary{shapes.geometric, arrows}

\pgfdeclarelayer{background}
\pgfsetlayers{background,main}  % 'background' drawn first, 'main' on top


% colors for the main blocks
\definecolor{offblue}{RGB}{102, 178, 255}
\definecolor{offred}{RGB}{255, 153, 51}
\definecolor{cutlergreen}{RGB}{0, 104, 72}
\definecolor{undertheelms}{RGB}{2, 66, 48 }
\definecolor{rust}{RGB}{250, 70, 22}
\definecolor{sycamore}{RGB}{231, 236, 195 }
% https://www.ohio.edu/ucm/ohio-brand/colors

% \tikzstyle{offlinestageblock} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=yellow!30]
% \tikzstyle{somename} = [ellipse, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=purple!30]
\tikzstyle{block} = [rectangle, minimum width=60px, minimum height=70px, text centered, draw=black, fill=yellow!30, fill opacity=1.0]
\tikzstyle{blueblock} = [rectangle, minimum width=60px, minimum height=70px, text centered, draw=black, 
fill=blue!10, fill opacity = 0.2]
\tikzstyle{redblock} = [rectangle, minimum width=60px, minimum height=70px, text centered, draw=black, fill=red!30, fill opacity=0.5]
\tikzstyle{importantblock} = [rectangle, minimum width=65px, minimum height=70px, text centered, draw=black, fill=red!30]
% \tikzstyle{additional} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=yellow!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{line} = [thick,--,>=stealth]


\def \blockwidth{64px}
\def \arrowdepth{-109px}

\def \wordheight{-13px}

\def \xpadding{2px}
\def \ypadding{3px}

\def \rectbottom{-118px}
\def \curveradius{8px}

\def \stepspacing{-12px}
\def \topypad{2px}

\definecolor{darkblue}{rgb}{0, 0, 0.25}
\definecolor{darkred}{rgb}{0.25, 0, 0}




\begin{tikzpicture}[node distance=72px]

\node (initial) [block, text width = \blockwidth, xshift=-12px - 6px, yshift=-62px, inner ysep=\ypadding, inner xsep=\xpadding]
{
% Step \#0 \vspace{\stepspacing} \\
\vspace{\topypad} \\
Place Initial Snapshot(s)
};
\node[above=\stepspacing of initial] 
{\textbf{Step 0}};


\node (scan) [block, right of=initial, text width = \blockwidth + 6px, xshift=7px + 3px, 
inner ysep=\ypadding,
inner xsep=\xpadding]
{
\vspace{\topypad} \\
Determine Parameter of Maximum Estimated Error
};
\node[above=\stepspacing of scan] 
{\textbf{Step 1}};


\node (additional) [block, right of=scan, text width=\blockwidth, xshift=7px + 3px, 
inner ysep=\ypadding,
inner xsep=\xpadding] 
{
\vspace{\topypad} \\
Compute FOM at Determined Parameter
};
\node[above=\stepspacing of additional] 
{\textbf{Step 2}};


\node (update) [block, right of=additional, text width=\blockwidth, xshift=7px, 
inner ysep=\ypadding,
inner xsep=\xpadding]
{
\vspace{\topypad} \\
Update \\ Emulator Offline Stage
};
\node[above=\stepspacing of update] 
{\textbf{Step 3}};


\node (check) [block, right of=update, xshift=7px, text width=\blockwidth, 
inner ysep=\ypadding,
inner xsep=\xpadding]
{
\vspace{\topypad} \\
Check\\Algorithm\\Break\\Conditions
};
\node[above=\stepspacing of check] 
{\textbf{Step 4}};


{};
\node (end1) [block, right of=check, text width = \blockwidth, xshift=18px, 
inner ysep=\ypadding,
inner xsep=6px]
{
    % Step \#5 \vspace{\stepspacing} \\
    Apply $\bm{\theta}$ onto \\Projections.
    \\
    \vspace{4px}
    Estimate Error (optional)
};




\draw [arrow] (initial) -- (scan);
\draw [arrow] (scan) -- (additional);
\draw [arrow] (additional) -- (update);
\draw [arrow] (update) -- (check);
% \draw [arrow] (update) -- (check);
\draw [arrow] (check) -- (end1);

\draw[thick] (check.south) -- (274px + 30px, \arrowdepth);
\draw[thick] (274px + 30px, \arrowdepth) -- (37px + 30px - 3px, \arrowdepth);
\draw [arrow] (37px + 30px - 3px, \arrowdepth) -- (scan.south);


% \begin{pgfonlayer}{background}
%     \fill[blue!20] (-60px, 0px) rectangle (345px, -112px);
%     \fill[red!20] (348px, 0px) rectangle (440px, -112px);
% \end{pgfonlayer}
\begin{pgfonlayer}{background}
    % \fill[cutlergreen!50] 
    \fill[blue!30] 
    (-60px, 0px) -- 
    (-60px + \curveradius, 0px) arc[start angle=90, end angle=180, radius=\curveradius] --
    (-60px, \rectbottom) -- 
    (-60px, \rectbottom + \curveradius) arc[start angle=180, end angle=270, radius=\curveradius] -- 
    (347px, \rectbottom) -- 
    (347px, 0px) --
    (-60px, 0px) -- 
    cycle;

    % \fill[rust!80]
    \fill[red!30]
    (347px, 0px) --
    (347px, \rectbottom) --
    (440px, \rectbottom) --  
    (440px - \curveradius, \rectbottom) arc[start angle=-90, end angle=0, radius=\curveradius] -- 
    (440px, 0px) --
    (440px, 0px - \curveradius) arc[start angle=0, end angle=90, radius=\curveradius] -- 
    cycle;
\end{pgfonlayer}




\node at (142.5px, \wordheight) [darkblue]
{\scalebox{1.6}{Offline Stage}};
\node at (395px, \wordheight) [darkred]
{\scalebox{1.6}{Online Stage}};


\end{tikzpicture}

==> figures/tikz/pod_vs_greedy.tex <==
% \documentclass{article}
% \usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{shapes.geometric, arrows}
% \usepackage{graphicx} % For including images

\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{box} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=yellow!30]

\def \yshift {-2.5}
\def \xshift {-1.33}

\begin{tikzpicture}


% Add a title as a node above the images
% \node at (0.25, 0) {\textbf{Greedy Iterations}};
\node at (4.3 + 0.3, 0) {\textbf{Greedy Algorithm}};

% First image node
% \node (greedy) at (0, -2.3)
\node (greedy) at (4.3, -2.3)
{\includegraphics[width=0.495 \columnwidth]
{greedy_6_with_green_dots.png}
};

\node (orth) 
[box, 
below of=greedy, 
text width = 100, 
xshift=10px,
yshift=-55px]
{Orthonormalization \\ 
%$
% \#\rm{HF}
% n_{\rm{HF}}
% \hspace{-6px}=\hspace{-6px}6$
(6 FOM samples)
};



% Add a title as a node above the images
% \node at (4 + 0.3, 0) {\textbf{POD Approach}};
\node (PODtitle) at (0.25, 0) {\textbf{POD Approach}};


% \node (pod) at (4, -2.3)
\node (pod) at (0, -2.3)
{\includegraphics[width=0.495 \columnwidth]
{pod.png}
};

\node (SVD) 
[box, 
below of=pod, 
text width = 100, 
xshift=8.5px,
yshift=-55px]
{Truncated SVD \\ 
%$
% \#\rm{HF}
%n_{\rm{HF}}
%\hspace{-6px}=\hspace{-6px}100$
(100 FOM samples)
};

\node (basis)
[box,
below of = orth,
text width = 100,
xshift = -67px,
yshift = -15px]
{Emulator Basis \\ ($n_b\hspace{-6px}=\hspace{-6px}6$)};




\draw [arrow] 
($(pod) + (0.3, -2.0)$)
to[out=270, in=90]
($(SVD) + (0, 0.52)$);

\draw [arrow] 
($(greedy) + (0.35, -2.0)$)
to[out=270, in=90]
($(orth) + (0, 0.52)$);

\draw [arrow]
($(SVD.270)$)
--
($(basis.90 + 70)$);
\draw [arrow]
($(orth.270)$)
--
($(basis.90 - 70)$);


\draw [arrow]
($(greedy) + (-0.94, -1.01)$)
to[out=120, in=150]
($(greedy) + (1.42, 1.55)$);
\draw [arrow]
($(greedy) + (1.50, 1.513)$)
to[out=-45, in=45]
($(greedy) + (1.68, -0.8)$);
\draw [arrow]
($(greedy) + (1.60, -0.8)$)
to[out=150, in=225]
($(greedy) + (1.735, 0.505)$);
\draw [arrow]
($(greedy) + (1.74, 0.555)$)
to[out=140, in=65]
($(greedy) + (-0.55, 0.25)$);
\draw [arrow]
($(greedy) + (-0.525, 0.19)$)
to[out=340, in=70]
($(greedy) + (0.14, -1.025)$);


% \node (SVD_nb) at (-12px, -15px) {$n_b = 100$};

% \node at (5.65, -1.73) {\scalebox{0.7}{\bm{$+$}}};
% \node at (5.4, -0.8) {\scalebox{0.7}{\bm{$+$}}};
% \node at (3.85, -2.6) {\scalebox{0.7}{\bm{$+$}}};
% \node at (5.15, -2.95) {\scalebox{0.7}{\bm{$+$}}};
% \node at (5.95, -2.2) {\scalebox{0.7}{\bm{$+$}}};

\end{tikzpicture}


==> figures/tikz/truncated-SVD.tex <==
% \documentclass{article}
% \usepackage{tikz}
% \usepackage{mathabx}
% \usepackage{bm}

\def \boxspacingone{91px}
\def \boxspacingtwo{139px}

\def \approxx{4px}
\def \approxy{5px}
\def \lowshift{-0.02}

\def \n{75px}
\def \m{45px}
\def \t{30px}



\begin{tikzpicture}
    
    % M
    \node
    [draw, fill=gray!70,
    minimum width=\m, minimum height=\n]
    (M) at (-25px, 0) 
    {};
    \node at (-25px, 15px) {\scalebox{1.4}{\textbf{M}}\,};
    \node at (-25px, 5px) {\scalebox{1.0}{$n \times m$}};
    
    % equal / approx sign
    \node at (8px, 15px) {\large \textbf{=}};
    % \node at (32px, 10px) { \approx };
    \begin{scope}[shift={(\approxx, \approxy)}]
        \draw [dash pattern=on 1.5pt off 1pt, thick] 
        plot[smooth, tension=1] 
        coordinates {(0, 0.05) 
                     (0.1, 0.15) 
                     (0.2, 0.05) 
                     (0.3, 0.15)};
    \draw [dash pattern=on 1.5pt off 1pt, thick] 
        plot[smooth, tension=1] 
        coordinates {(0, -0.05 + \lowshift) 
                     (0.1, 0.05 + \lowshift) 
                     (0.2, -0.05 + \lowshift) 
                     (0.3, 0.05 + \lowshift)};
    \end{scope}

    
    % U
    \node
    [draw, fill=blue!60, right of = M,
    minimum width=\n, minimum height=\n]
    (U) at (28px, 0) 
    {};
    \node
    [draw, dashed, fill=blue!20, right of = M,
    minimum width=\t-2px, minimum height=\n - 2px, 
    fill opacity = 0.5] 
    (Utruncated) at (6px, 0px) 
    {};
    
    \node (Utext) at (72px, -5px) {\scalebox{1.4}{$\bm{U}$}};
    \node[anchor=north] at ($(Utext.south) - (0, 2px)$) {\scalebox{1.0}{$n \times n$}};
    
    \node (Urtext) at (34px, 25px - 4px) {\,\scalebox{1.4}{$\bm{U}_r$}};
    \node[anchor=north] at ($(Urtext.south) - (0, 2px)$) {\scalebox{1.0}{$n \times r$}};


    % Sigma
    \node
    [draw, fill=orange!60, right of = U,
    minimum width=\m, minimum height=\n]
    (Sigma) at (\boxspacingone, 0) 
    {};
    \node
    [draw, dashed, fill=orange!20, right of = U,
    minimum width=\t-2px, minimum height=\t - 2px, 
    fill opacity = 0.5] 
    (Sigmatruncated) at (\boxspacingone - 7px, 22px) 
    {};

    \node (Sigmatext) at (120px, -5px) {\scalebox{1.4}{$\bm{\Sigma}$}};
    \node[anchor=north] at ($(Sigmatext.south) - (0, 2px)$) {\scalebox{1.0}{$n \times m$}};
    
    \node (Sigmartext) at (112px, 25px) {\,\,\scalebox{1.4}{$\bm{\Sigma}_r$}};
    \node[anchor=north] at ($(Sigmartext.south) - (0, 2px)$) {\scalebox{1.0}{$r \times r$}};

    % V transpose
    \node
    [draw, fill=green!60, right of = Simga,
    minimum width=\m, minimum height=\m]
    (V) at (\boxspacingtwo, 15px) 
    {};
    \node
    [draw, dashed, fill=green!20, right of = Sigma,
    minimum width=\m-2px, minimum height=\t - 2px, 
    fill opacity = 0.5] 
    (Vtruncated) at (\boxspacingtwo, 22px) 
    {};

    \node (Vtext) at (176px, -15px) {\scalebox{1.4}{$\bm{V^\dagger}$}};
    \node[anchor=north] at ($(Vtext.south) - (0, 2px)$) {\scalebox{1.0}{$m \times m$}};
    
    \node (Vrtext) at (168px, 25px) {\,\,\scalebox{1.4}{$\bm{V^\dagger}_r$}};
    \node[anchor=north] at ($(Vrtext.south) - (0, 2px)$) {\scalebox{1.0}{$r \times m$}};

\end{tikzpicture}

